Denoising-based UNMT is more robust to word-order divergence than MASS-based UNMT

We aim to investigate whether UNMT approaches with self-supervised pre-training are robust to word-order divergence between language pairs. We achieve this by comparing two models pre-trained with the same self-supervised pre-training objective. The first model is trained on language pairs with different word-orders, and the second model is trained on the same language pairs with source language re-ordered to match the word-order of the target language. Ideally, UNMT approaches which are robust to word-order divergence should exhibit no visible performance difference between the two configurations. In this paper, we investigate two such self-supervised pre-training based UNMT approaches, namely Masked Sequence-to-Sequence Pre-Training, (MASS) (which does not have shuffling noise) and Denoising AutoEncoder (DAE), (which has shuffling noise). We experiment with five English$\rightarrow$Indic language pairs, i.e., en-hi, en-bn, en-gu, en-kn, and en-ta) where word-order of the source language is SVO (Subject-Verb-Object), and the word-order of the target languages is SOV (Subject-Object-Verb). We observed that for these language pairs, DAE-based UNMT approach consistently outperforms MASS in terms of translation accuracies. Moreover, bridging the word-order gap using reordering improves the translation accuracy of MASS-based UNMT models, while it cannot improve the translation accuracy of DAE-based UNMT models. This observation indicates that DAE-based UNMT is more robust to word-order divergence than MASS-based UNMT. Word-shuffling noise in DAE approach could be the possible reason for the approach being robust to word-order divergence.

==> acc.tex <==
\begin{comment}
 

\begin{table*}[ht!]
    \centering
    \resizebox{\textwidth}{!}{ 
    \begin{tabular}{l | rr |rr| rr| rr| rr|}
    \toprule
     \textbf{UNMT}  & \multicolumn{2}{c|}{en - hi}   & \multicolumn{2}{c|}{en - bn} & \multicolumn{2}{c|}{en - gu} & \multicolumn{2}{ c|}{en - kn}  & \multicolumn{2}{ c|}{en - ta} \\
     \cline{2-11}
     \textbf{approaches} 
    & S $\rightarrow$ T & T  $\rightarrow$ S & S $\rightarrow$ T & T  $\rightarrow$ S & S $\rightarrow$ T & T  $\rightarrow$ S & S $\rightarrow$ T & T  $\rightarrow$ S & S $\rightarrow$ T & T  $\rightarrow$ S\\ 
    \midrule
     MASS-static &  6.69 & 7.04 & 1.63 & 3.38 & 3.96 & 5.36 & 2.22 & 4 & 1.47 & 3.03\\
     MASS-static + R &   \textbf{11.62} & \textbf{12.01} & \textbf{2.37} & \textbf{4.27} & \textbf{5.88} & \textbf{8.09} & \textbf{3.34} & \textbf{6.2} & \textbf{2.1} & \textbf{4.37} \\
    \midrule
    DAE-static &  9.54 & 9.91 & 2.14 & 3.24 & 5.68 & 7.33 & 2.94 & 5.78 & 1.7 & 4.35  \\
    DAE-static + R & \textbf{13.41} & \textbf{14.16} & \textbf{3.1} & \textbf{4.95} & \textbf{7.85} & \textbf{11.01} & \textbf{3.59} & \textbf{6.58} & \textbf{2.23} & \textbf{6.39}  \\
    \bottomrule
    \end{tabular}
    }
    \caption{Translation accuracies at first epoch of finetuning of MASS-pretrained and DAE-pretained UNMT models for distant languages, i.e. en-hi, en-bn, en-gu, en-kn, en-ta test sets (BLEU scores reported). The values marked in bold indicate the best score for each language pair and each LM approach. }
    \label{resultft0}
    
\end{table*}
\end{comment}


\begin{comment}
 \begin{table*}[ht!]
    \centering
    \resizebox{\textwidth}{!}{ 
    \begin{tabular}{|l | rr |rr| rr| rr| rr|}
    \toprule
     \textbf{UNMT}  & \multicolumn{2}{c|}{en - hi}   & \multicolumn{2}{c|}{en - bn} & \multicolumn{2}{c|}{en - gu} & \multicolumn{2}{ c|}{en - kn}  & \multicolumn{2}{ c|}{en - ta} \\
     \cline{2-11}
     \textbf{approaches} 
    & S $\rightarrow$ T & T  $\rightarrow$ S & S $\rightarrow$ T & T  $\rightarrow$ S & S $\rightarrow$ T & T  $\rightarrow$ S & S $\rightarrow$ T & T  $\rightarrow$ S & S $\rightarrow$ T & T  $\rightarrow$ S\\ 
    \midrule
     MASS-static &  &   & & & & &&&&  \\
     MASS-static + R &  &   & & & & &&&&\\
    \midrule
    DAE-static &   &   & & & & &&&& \\
    DAE-static + R &  &   & & & & &&&&\\
    \bottomrule
    \end{tabular}
    }
    \caption{Translation accuracies of MASS-pretrained and DAE-pretained UNMT models for distant languages, i.e. en-hi, en-bn, en-gu, en-kn, en-ta test sets (BLEU scores reported). The values marked in bold indicate the best score for each language pair and each LM approach .}
    \label{result}
    
\end{table*}
\end{comment}
 
\begin{table*}[ht!]
    \centering
    \resizebox{\textwidth}{!}{ 
    \begin{tabular}{l | rr |rr| rr| rr| rr }
    \toprule
     \textbf{UNMT}  & \multicolumn{2}{c|}{en - hi}   & \multicolumn{2}{c|}{en - bn} & \multicolumn{2}{c|}{en - gu} & \multicolumn{2}{ c|}{en - kn}  & \multicolumn{2}{ c }{en - ta} \\
     \cline{2-11}
     \textbf{approaches} 
    & S $\rightarrow$ T & T  $\rightarrow$ S & S $\rightarrow$ T & T  $\rightarrow$ S & S $\rightarrow$ T & T  $\rightarrow$ S & S $\rightarrow$ T & T  $\rightarrow$ S & S $\rightarrow$ T & T  $\rightarrow$ S\\ 
    \midrule
     MASS-static & 39.5 & 46.1 & 25.4 & 29.6 & 31.1 & 36.9 & 30.7 & 33.8 & 31.4 & 28.7 \\
     MASS-static + R & 41.8 & 47.5 & 28.9 & 35.5 & 37.5 & 43.7 & 36.5 & 39.9 & 34.3 & 33 \\
    \midrule
    DAE-static & 45.6 & 52.2 & 28.4 & 34.6 & 38.5 & 45.7 & 35.9 & 40.3 & 33 & 34.5 \\
    DAE-static + R &  42.2 & 48 & 29.6 & 36.2 & 37.6 & 44.2 & 36.5 & 39.6 & 35.5 & 36 \\
    \bottomrule
    \end{tabular}
    }
    \caption{Translation accuracies of MASS-pretrained and DAE-pretained UNMT models with/without Reordering (R) for distant languages, i.e. en-hi, en-bn, en-gu, en-kn, en-ta test sets (ChrF scores reported). The values marked in bold indicate the best score for each language pair and each LM approach. }
    \label{resultchrf}
    
\end{table*}


\begin{table*}[ht!]
    \centering
    \resizebox{\textwidth}{!}{ 
    \begin{tabular}{l | rr |rr| rr| rr| rr }
    \toprule
     \textbf{UNMT}  & \multicolumn{2}{c|}{en - hi}   & \multicolumn{2}{c|}{en - bn} & \multicolumn{2}{c|}{en - gu} & \multicolumn{2}{ c|}{en - kn}  & \multicolumn{2}{ c }{en - ta} \\
     \cline{2-11}
     \textbf{approaches} 
    & S $\rightarrow$ T & T  $\rightarrow$ S & S $\rightarrow$ T & T  $\rightarrow$ S & S $\rightarrow$ T & T  $\rightarrow$ S & S $\rightarrow$ T & T  $\rightarrow$ S & S $\rightarrow$ T & T  $\rightarrow$ S\\ 
    \midrule
     MASS-static & 14.2 & 14 & 1.5 & 2.8 & 5.3 & 6.3 & 3.1 & 5.1 & 1.8 & 2.7 \\
     MASS-static + R & 14.6 & - & 3 & - & 8.6 & - & 4.5 & - & 2.6 & - \\
    \midrule
    DAE-static & \textbf{21} & \textbf{21.9} & 2.9 & \textbf{4.4} & \textbf{10.6} & \textbf{14.8} & 4.4 & \textbf{9.4} & 2.5 & \textbf{4.8} \\
    DAE-static + R &  15.2 & - & \textbf{3.3} & - & 8.7 & - & 4.2 & - & 2.7 & -\\
    \bottomrule
    \end{tabular}
    }
    \caption{Translation accuracies of MASS-pretrained and DAE-pretained UNMT models with/without Reordering (R) for distant languages, i.e. en-hi, en-bn, en-gu, en-kn, en-ta test sets (BLEU scores reported). The values marked in bold indicate the best score for each language pair and each LM approach. }
    \label{result}
    
\end{table*}


\begin{table*}[ht!]
    \centering
    \resizebox{\textwidth}{!}{ 
    \begin{tabular}{l | rr |rr| rr| rr| rr }
    \toprule
     \textbf{UNMT}  & \multicolumn{2}{c|}{en - hi}   & \multicolumn{2}{c|}{en - bn} & \multicolumn{2}{c|}{en - gu} & \multicolumn{2}{ c|}{en - kn}  & \multicolumn{2}{ c }{en - ta} \\
     \cline{2-11}
     \textbf{approaches} 
    & S $\rightarrow$ T & T  $\rightarrow$ S & S $\rightarrow$ T & T  $\rightarrow$ S & S $\rightarrow$ T & T  $\rightarrow$ S & S $\rightarrow$ T & T  $\rightarrow$ S & S $\rightarrow$ T & T  $\rightarrow$ S\\ 
    \midrule
     MASS-static & 39.5 & 46.1 & 25.4 & 29.6 & 31.1 & 36.9 & 30.7 & 33.8 & 31.4 & 28.7 \\
     MASS-static + R & 41.8 & - & 28.9 & - & 37.5 & - & 36.5 & - & 34.3 & - \\
    \midrule
    DAE-static & 45.6 & 52.2 & 28.4 & 34.6 & 38.5 & 45.7 & 35.9 & 40.3 & 33 & 34.5 \\
    DAE-static + R &  42.2 & - & 29.6 & - & 37.6 & - & 36.5 & - & 35.5 & - \\
    \bottomrule
    \end{tabular}
    }
    \caption{Translation accuracies of MASS-pretrained and DAE-pretained UNMT models with/without Reordering (R) for distant languages, i.e. en-hi, en-bn, en-gu, en-kn, en-ta test sets (ChrF scores reported). The values marked in bold indicate the best score for each language pair and each LM approach. }
    \label{resultchrf}
    
\end{table*}


\begin{comment} 
\begin{table*}[ht!]
    \centering
    \resizebox{\textwidth}{!}{ 
    \begin{tabular}{ll  rr rr rr rr rr }
    \toprule
     \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Evaluation\\ metric\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}UNMT\\ Approach\end{tabular}}} & \multicolumn{2}{c}{en - hi}   & \multicolumn{2}{c}{en - bn} & \multicolumn{2}{c}{en - gu} & \multicolumn{2}{ c}{en - kn}  & \multicolumn{2}{ c }{en - ta} \\
     \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10} \cmidrule(lr){11-12}
      &  
    & S $\rightarrow$ T & T  $\rightarrow$ S & S $\rightarrow$ T & T  $\rightarrow$ S & S $\rightarrow$ T & T  $\rightarrow$ S & S $\rightarrow$ T & T  $\rightarrow$ S & S $\rightarrow$ T & T  $\rightarrow$ S\\ 
    % \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6} \cmidrule(lr){7-7} \cmidrule(lr){8-8} \cmidrule(lr){9-9} \cmidrule(lr){10-10} \cmidrule(lr){11-11} \cmidrule(lr){12-12}
    \midrule
     \multirow{4}{*}{BLEU} & MASS-static & 14.2 & 14 & 1.5 & 2.8 & 5.3 & 6.3 & 3.1 & 5.1 & 1.8 & 2.7 \\
     & MASS-static + R & 14.6 & - & 3 & - & 8.6 & - & \textbf{4.5} & - & 2.6 & - \\
    \cmidrule{2-12}
    & DAE-static & \textbf{21} & \textbf{21.9} & 2.9 & \textbf{4.4} & \textbf{10.6} & \textbf{14.8} & 4.4 & \textbf{9.4} & 2.5 & \textbf{4.8} \\
    & DAE-static + R &  15.2 & - & \textbf{3.3} & - & 8.7 & - & 4.2 & - & \textbf{2.7} & -\\
    \midrule
    \multirow{4}{*}{ChrF} & MASS-static & 39.5 & 46.1 & 25.4 & 29.6 & 31.1 & 36.9 & 30.7 & 33.8 & 31.4 & 28.7 \\
     & MASS-static + R & 41.8 & - & 28.9 & - & 37.5 & - & \textbf{36.5} & - & 34.3 & - \\
    \cmidrule{2-12}
    & DAE-static & \textbf{45.6} & \textbf{52.2} & 28.4 & \textbf{34.6} & \textbf{38.5} & \textbf{45.7} & 35.9 & \textbf{40.3} & 33 & \textbf{34.5} \\
    & DAE-static + R &  42.2 & - & \textbf{29.6} & - & 37.6 & - & \textbf{36.5} & - & \textbf{35.5} & - \\
    \bottomrule
    \end{tabular}
    }
    \caption{Translation accuracies of MASS-pretrained and DAE-pretained UNMT models with/without Reordering (R) for distant language-pairs, i.e. en-hi, en-bn, en-gu, en-kn, en-ta in both S $\rightarrow$ T and T  $\rightarrow$ S directions (S and T refers to source and target). The values marked in bold indicate the best scores for each language pair.}
    \label{result}
    
\end{table*}
\end{comment}

==> inputs/related.tex <==
lexical divergence handling papers

tallip word order


\resizebox{\textwidth}{!}{ 
    \begin{tabular}{ll  ll ll ll ll ll }
    \toprule
     \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Evaluation\\ metric\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}UNMT\\ Approach\end{tabular}}} & \multicolumn{2}{c}{en - hi}   & \multicolumn{2}{c}{en - bn} & \multicolumn{2}{c}{en - gu} & \multicolumn{2}{ c}{en - kn}  & \multicolumn{2}{ c }{en - ta} \\
     \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10} \cmidrule(lr){11-12}
      &  
    & S $\rightarrow$ T & T  $\rightarrow$ S & S $\rightarrow$ T & T  $\rightarrow$ S & S $\rightarrow$ T & T  $\rightarrow$ S & S $\rightarrow$ T & T  $\rightarrow$ S & S $\rightarrow$ T & T  $\rightarrow$ S\\  
    \midrule
     \multirow{4}{*}{BLEU} & MASS-static & 14.16 & 14.03 & 1.51 & 2.77 & 5.31 & 6.25 & 3.08 & 5.11 & 1.81 & 2.70  \\
     & MASS-static + R &  14.63 ($\uparrow$ 0.47) & - & 3.04 ($\uparrow$ 1.53) & - & 8.62 ($\uparrow$ 3.31) & - & \textbf{4.48} ($\uparrow$ 1.4) & - & 2.57 ($\uparrow$ 0.76) & - \\
    \cmidrule{2-12}
    & DAE-static &  \textbf{21.03} & \textbf{21.89} & 2.88 & \textbf{4.39} & \textbf{10.60} & \textbf{14.78} & 4.42 & \textbf{9.40} & 2.52 & \textbf{4.77} \\
    & DAE-static + R & 15.22   ($\downarrow$5.81) & - & \textbf{3.27} ($\uparrow$ 0.39) & - & 8.72 ($\downarrow$ 1.88) & - & 4.18 ($\downarrow$ 0.24) & - & \textbf{2.65} ($\uparrow$ 0.13) & -  \\
    \midrule
    \multirow{4}{*}{ChrF} & MASS-static &  39.45 & 46.07 & 25.39 & 29.56 & 31.08 & 36.87 & 30.73 & 33.83 & 31.40 & 28.73 \\
     & MASS-static + R & 41.77 ($\uparrow$ 2.32) & - & 28.85 ($\uparrow$ 3.46) & - & 37.45 ($\uparrow$ 6.37) & - & \textbf{36.47} ($\uparrow$ 5.74) & - & 34.34 ($\uparrow$ 2.94) & - \\
    \cmidrule{2-12}
    & DAE-static &  \textbf{45.63} & \textbf{52.21} & 28.36 & \textbf{34.61} & \textbf{38.55} & \textbf{45.74} & 35.89 & \textbf{40.33} & 33.00 & \textbf{34.48} \\
    & DAE-static + R &  42.18 ($\downarrow$ 3.45) & - & \textbf{29.65} ($\uparrow$ 1.29) & - & 37.58 ($\downarrow$ 0.97) & - & 36.46 ($\uparrow$ 0.57) & - & \textbf{35.52} ($\uparrow$ 2.52) & - \\
    \bottomrule
